MagicEdit: High-Fidelity and Temporally Coherent Video Editing

In this report, we present MagicEdit, a surprisingly simple yet effective solution to the text-guided video editing task. We found that high-fidelity and temporally coherent video-to-video translation can be achieved by explicitly disentangling the learning of content, structure and motion signals during training. This is in contradict to most existing methods which attempt to jointly model both the appearance and temporal representation within a single framework, which we argue, would lead to degradation in per-frame quality. Despite its simplicity, we show that MagicEdit supports various downstream video editing tasks, including video stylization, local editing, video-MagicMix and video outpainting.

==> Makefile <==
main:
	pdflatex main

full:
	pdflatex main && \
	bibtex main && \
	pdflatex main && \
	pdflatex main

cut: full
	pdftk main.pdf cat 1-10 output paper.pdf
	pdftk main.pdf cat 11-end 9-10 output supp.pdf

clean:
	rm *.aux *.bbl *.blg *.log *.pdf *.dep *.brf *.fls *.out

